Analyzing the Performance of Multilayer Neural Networks for Object Recognition

In the last two years, convolutional neural networks (CNNs) have achieved an impressive suite of results on standard recognition datasets and tasks. CNN-based features seem poised to quickly replace engineered representations, such as SIFT and HOG. However, compared to SIFT and HOG, we understand much less about the nature of the features learned by large CNNs. In this paper, we experimentally probe several aspects of CNN feature learning in an attempt to help practitioners gain useful, evidence-backed intuitions about how to apply CNNs to computer vision problems.

==> texfiles/methods.tex <==
\section{Experimental setup}
\label{sec:train}

\subsection{Datasets and tasks}
In this paper, we report experimental results using several standard datasets and tasks, which we summarize here.

\subsubsection{Image classification.} For the task of image classification we consider two datasets, the first of which is PASCAL VOC 2007 \cite{Pascal}.
We refer to this dataset and task by ``PASCAL-CLS''.
Results on PASCAL-CLS are reported using the standard average precision (AP) and mean average precision (mAP) metrics.

PASCAL-CLS is fairly small-scale with only 5k images for training, 5k images for testing, and 20 object classes.
Therefore, we also consider the medium-scale SUN dataset \cite{sun}, which has around 108k images and 397 classes.
We refer to experiments on SUN by ``SUN-CLS''.
In these experiments, we use a non-standard train-test split since it was computationally infeasible to run all of our experiments on the 10 standard subsets proposed by \cite{sun}. 
Instead, we randomly split the dataset into three parts (train, val, and test) using 50\%, 10\% and 40\% of the data, respectively. 
The distribution of classes was uniform across all the three sets.
We emphasize that results on these splits are only used to support investigations into properties of CNNs and not for comparing against other scene-classification methods in the literature.
For SUN-CLS, we report 1-of-397 classification accuracy averaged over all classes, which is the standard metric for this dataset.
For select experiments we report the error bars in performance as mean $\pm$ standard deviation in accuracy over 5 runs (it was computationally infeasible to compute error bars for all experiments). For each run, a different random split of train, val, and test sets was used.  

\subsubsection{Object detection.} For the task of object detection we use PASCAL VOC 2007.
We train using the trainval set and test on the test set.
We refer to this dataset and task by ``PASCAL-DET''.
PASCAL-DET uses the same set of images as PASCAL-CLS.
We note that it is standard practice to use the 2007 version of PASCAL VOC for reporting results of ablation studies and hyperparameter sweeps.
We report performance on PASCAL-DET using the standard AP and mAP metrics.
In some of our experiments we use only the ground-truth PASCAL-DET bounding boxes, in which case we refer to the setup by ``PASCAL-DET-GT''.

In order to provide a larger detection training set for certain experiments, we also make use of the ``PASCAL-DET+DATA'' dataset, which we define as including VOC 2007 trainval union with VOC 2012 trainval.
The VOC 2007 test set is still used for evaluation.
This dataset contains approximately 37k labeled bounding boxes, which is roughly three times the number contained in PASCAL-DET.

\subsection{Network architecture and layer nomenclature}
\label{sub:net-arch}
All of our experiments use a single CNN architecture.
This architecture is the Caffe \cite{caffe} implementation of the network proposed by Krizhevsky et al. \cite{Kriz}.
The layers of the CNN are organized as follows.
The first two are subdivided into four sublayers each: convolution (conv), $\max(x,0)$ rectifying non-linear units (ReLUs), max pooling, and local response normalization (LRN). 
Layers 3 and 4 are composed of convolutional units followed by ReLUs.
Layer 5 consists of convolutional units, followed by ReLUs and max pooling.
The last two layers are fully connected (fc). 
When we refer to conv-1, conv-2, and conv-5 we mean the output of the max pooling units following the convolution and ReLU operations (also following LRN when applicable).\footnote{Note that this nomenclature differs slightly from \cite{Rcnn}.}
For layers conv-3, conv-4, fc-6, and fc-7 we mean the output of ReLU units.
%FT or FT-Net refers to a finetuned network whereas as FC-FT or FC-FT-Net refers to a network finetuned by setting the learning rate of the first 5 layers to zero. We use the terms CNNs and ConvNets interchangeably to refer to multilayer network architectures of the type proposed in \cite{Kriz}. Terms filter/unit are used interchangeably to refer to filters of the CNN and GT-BBOX/gt-bbox stands for Ground truth bounding boxes from the PASCAL-VOC-2007 detection challenge and mAP refers to mean average precision \cite{Pascal}.

%\subsection{Training Setup} 
%\label{sub:train-setup}
%Results for image and GT-BBOX classification were obtained by training linear SVMs on train-val sets of PASCAL-VOC-2007 \cite{Pascal} and tested on the test set. For detection we closely follow the RCNN setup described in \cite{Rcnn}. For SUN-397 \cite{sun} we used a non-standard train-test splits since it was infeasible to finetune CNNs for 10 standard subsets proposed by \cite{sun}. Instead, we randomly split the dataset into 3 parts namely train,val and test using 50\%,10\% and 40\% of the data. The distribution of classes was uniform across all the 3 sets. Results on these splits are only used to support investigations into properties of CNNs and not for comparing against other scene-classification methods.  
 
\subsection{Supervised pre-training and fine-tuning}
\label{sub:fine-train}
Training a large CNN on a small dataset often leads to catastrophic overfitting.
%The idea of supervised pre-training is to use a data-rich auxiliary dataset and task, such as ImageNet classification, to initialize the CNN parameters before training models on a small dataset.
%This procedure is called \emph{fine-tuning}.
The idea of supervised \emph{pre-training} is to use a data-rich auxiliary dataset and task, such as ImageNet classification, to initialize the CNN parameters. 
The CNN can then be used on the small dataset, directly, as a feature extractor (as in \cite{Decaf}).
Or, the network can be updated by continued training on the small dataset, a process called \emph{fine-tuning}.
%The R-CNN object detection work in \cite{Rcnn} demonstrated that fine-tuning is an effective strategy for training object detectors.
%\cite{Decaf} also demonstrated that such pre-training, even without fine-tuning, can lead to state-of-the-art results on various image classification tasks. 

%We employ the supervised pre-training, domain-specific fine-tuning paradigm used by R-CNN \cite{Rcnn} in many experiments.
%The idea of supervised pre-training is to use a data-rich auxiliary dataset and task, such as ImageNet classification, to initialize a CNN with large number of parameters before training on a small dataset. Such initialization procedure allows the network parameters to be modified to achieve good performance on a small dataset without overfitting the large network to it.
%This procedure allows the small dataset to be used while avoiding disastrously overfitting the large network to it.
%For experiments in which the network is pre-trained on ImageNet, stochastic gradient descent is run for 310000 iterations (66 epochs).

For fine-tuning, we follow the procedure described in \cite{Rcnn}.
First, we remove the CNN's classification layer, which was specific to the pre-training task and is not reusable.
Next, we append a new randomly initialized classification layer with the desired number of output units for the target task.
Finally, we run stochastic gradient descent (SGD) on the target loss function, starting from a learning rate set to $0.001$ ($1/10$-th the initial learning rate used for training the network for ImageNet classification). 
%This choice was made to prevent clobbering the CNN's initialization.
This choice was made to prevent clobbering the CNN's initialization to control overfitting. 
%This choice was made to ensure that the network parameters don't overfit CNN's initialization.
At every 20,000 iterations of fine-tuning we reduce the learning rate by a factor of 10.

%\subsection{Method of Entropy Computation}
%\label{sub:def-ent}
%We define the entropy of a filter with respect to a given set of image-label pairs in the following way. Each image, when passed through the convolutional neural network produces a $p \times p$ heatmap of filter responses. (e.g. p = 6, for a layer 5 filter). We vectorize this heatmap into a vector of scores of length $p^2$ and with each element of this vector we associate the class label of the image. Thus, for each image we have a score vector and a label vector of length $p^2$ each. Next, we concatenate score vectors and label vectors from N images into a giant score vector and a giant label vector  of size $Np^2$ each. Now for every score threshold we consider all the labels which have an associated score $\geq$ to this threshold score. The entropy of this set of labels is the entropy of the filter at this threshold. As this threshold changes, entropy traces out a curve which we call as the entropy curve.  


==> texfiles/pretrain_finetune.tex <==
\section{The effects of fine-tuning and pre-training on CNN performance and parameters}
\label{sec:fine}
The results in \cite{Rcnn} (R-CNN) show that supervised pre-training for ImageNet classification, followed by fine-tuning for PASCAL object detection, leads to large gains over directly using features from the pre-trained network (without fine-tuning).
However, \cite{Rcnn} did not investigate three important aspects of fine-tuning: (1) What happens if we train the network ``from scratch'' (i.e., from a random initialization) on the detection data? (2) How does the amount of fine-tuning data change the picture? and (3) How does fine-tuning alter the network's parameters?
In this section, we explore these questions on object detection and image classification datasets.

\subsection{Effect of fine-tuning on CNN performance}
\label{sub:fine-performance}
\setlength{\tabcolsep}{2pt}
\begin{table}[t!]
\begin{center}
\caption{Comparing the performance of CNNs trained from scratch, pre-trained on ImageNet, and fine-tuned. PASCAL-DET+DATA includes additional data from VOC 2012 trainval. (Bounding-box regression was not used for detection results.)}
\vspace{0.3em}
\label{table:fine-effect}
\scalebox{0.95}{
\begin{tabular}{ccc|ccc|ccc}
\multicolumn{3}{c|}{\textbf{SUN-CLS}} & \multicolumn{3}{c|}{\textbf{PASCAL-DET}} & \multicolumn{3}{c}{\textbf{PASCAL-DET+DATA}} \\
scratch & pre-train & fine-tune  & scratch & pre-train & fine-tune & scratch & pre-train & fine-tune\\
\hline
$40.4 \pm 0.2$ & $53.1 \pm 0.2$ & $56.8 \pm 0.2$ & 40.7 & 45.5 & 54.1 & 52.3 & 45.5 & 59.2 \\ 
\end{tabular}}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}
The main results of this section are presented in Table \ref{table:fine-effect}.
First, we focus on the detection experiments, which we implemented using the open source R-CNN code.
All results use features from layer fc-7.

Somewhat surprisingly, it's possible to get reasonable results (40.7\% mAP) when training the CNN from scratch using only the training data from VOC 2007 trainval (13k bounding box annotations).
However, this is still worse than using the pre-trained network, directly, without fine-tuning (45.5\%).
Even more surprising is that when the VOC 2007 trainval data is augmented with VOC 2012 data (an additional 25k bounding box annotations), we are able to achieve a mAP of 52.3\% from scratch.
This result is almost as good as the performance achieved by pre-training on ImageNet and then fine-tuning on VOC 2007 trainval (54.1\% mAP).
These results can be compared to the 30.5\% mAP obtained by DetectorNet \cite{szegedy2013deep}, a recent detection system based on the same network architecture, which was trained from scratch on VOC 2012 trainval.

Next, we ask if ImageNet pre-training is still useful in the PASCAL-DET +DATA setting?
Here we see that even though it's possible to get good performance when training from scratch, pre-training still helps considerably.
The final mAP when fine-tuning with the additional detection data is 59.2\%, which is 5 percentage points higher than the best result reported in \cite{Rcnn} (both without bounding-box regression).
This result suggests that R-CNN performance is not data saturated and that simply adding more detection training data without any other changes may substantially improve results.

We also present results for SUN image classification.
Here we observe a similar trend: reasonable performance is achievable when training from scratch, however initializing from ImageNet and then fine-tuning yields significantly better performance.

\subsection{Effect of fine-tuning on CNN parameters}
\label{sub:fine-entropy}
We have provided additional evidence that fine-tuning a discriminatively pre-trained network is very effective in terms of task performance.
Now we look inside the network to see how fine-tuning changes its parameters.

To do this, we define a way to measure the class selectivity of a set of filters.
Intuitively, we use the class-label entropy of a filter given its activations, above a threshold, on a set of images.
Since this measure is entropy-based, a low value indicates that a filter is highly class selective, while a large value indicates that a filter fires regardless of class.
The precise definition of this measure is given in the Appendix.

In order to summarize the class selectivity for a \emph{set} of filters, we sort them from the most selective to least selective and plot the average selectivity of the first $k$ filters while sweeping $k$ down the sorted list.
Figure \ref{fig:fine-entropy} shows the class selectivity for the sets of filters in layers 1 to 7 before and after fine-tuning (on VOC 2007 trainval).
Selectivity is measured using the ground truth boxes from PASCAL-DET-GT instead of a whole-image classification task to ensure that filter responses are a direct result of the presence of object categories of interest and not correlations with image background.

\begin{comment}
\begin{figure}[t!]
\centering
\subfloat{\includegraphics[height=6.5cm]{images/ent_hist.png}}
\caption{Distribution of AuE for different layers in Alex-Net and FT-Net. X-axis is the entropy and the Y-axis is the number of filters. Notice that the left tail for fc-6 and fc-7 becomes heavier after finetuning. This indicates that finetuning makes these filters more discriminative.}
\label{fig:fine-hist}
\end{figure}
\end{comment}

\begin{figure}[t!]
\centering
\subfloat{\includegraphics[scale=0.20]{MCAUE.pdf}}
\caption{PASCAL object class selectivity plotted against the fraction of filters, for each layer, before fine-tuning (dash-dot line) and after fine-tuning (solid line). A lower value indicates greater class selectivity. Although layers become more discriminative as we go higher up in the network, fine-tuning on limited data (PASCAL-DET) only significantly affects the last two layers (fc-6 and fc-7).}
\label{fig:fine-entropy}
\end{figure}

\setlength{\tabcolsep}{2pt}
\begin{table}[t!]
\begin{center}
\caption{Comparison in performance when fine-tuning the entire network (ft) versus only fine-tuning the fully-connected layers (fc-ft).}
\label{table:fine-fc-ft}
\vspace{0.3em}
\scalebox{1}{
\begin{tabular}{cc|cc|cc}
\multicolumn{2}{c|}{\textbf{SUN-CLS}} & \multicolumn{2}{c|}{\textbf{PASCAL-DET}} & \multicolumn{2}{c}{\textbf{PASCAL-DET+DATA}} \\
ft & fc-ft  & ft & fc-ft & ft & fc-ft \\
\hline
$56.8 \pm 0.2$ & $56.2 \pm 0.1$ & 54.1 & 53.3 & 59.2 & 56.0 \\ 
\end{tabular}}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

Figure \ref{fig:fine-entropy} shows that class selectivity increases from layer 1 to 7 both with and without fine-tuning.
%This result is consistent with performance numbers reported in Table \ref{table:det-traj-classify}. 
It is interesting to note that entropy changes due to fine-tuning are only significant for layers 6 and 7. 
This observation indicates that fine-tuning only layers 6 and 7 may suffice for achieving good performance when fine-tuning data is limited. 
We tested this hypothesis on SUN-CLS and PASCAL-DET by comparing the performance of a fine-tuned network (ft) with a network which was fine-tuned by only updating the weights of fc-6 and fc-7 (fc-ft). 
These results, in Table \ref{table:fine-fc-ft}, show that with small amounts of data, fine-tuning amounts to ``rewiring'' the fully connected layers.
However, when more fine-tuning data is available (PASCAL-DET+DATA), there is still substantial benefit from fine-tuning all network parameters.

%We find that the final performance in the detection setup only drops by 0.8 points and by 0.6 points for scene-classification.  

%\setlength{\tabcolsep}{1pt}
%\begin{table}[t!]
%\begin{center}
%\caption{\todo{Include layer-wise results for PASCAL-DET-2?} for Evaluation of effect finetuning towards the task of object detection. (l5, l6, l7: layers 5, 6 and 7 of Alex Net)}
%\label{table:det-fine}
%\scalebox{0.75}{
%\begin{tabular}{l|cccccccccccccccccccc||c}
%\hline\noalign{\smallskip}
%layer & aero & bike & bird & boat & bottle & bus & car & cat & chair & cow & table & dog & horse & mbike & person & plant & sheep & sofa & train & tv & mAP \\
%\noalign{\smallskip}
%\hline
%l5 & 51.9 & 61.1 & 36.8 & 28.4 & 23.7 & 52.3 & 60.8 & 48.4 & 24.9 & 47.1 & 47.5 & 42.1 & 55.6 & 58.7 & 42.5 & 24.5 & 46.9 & 39.3 & 52.0 & 55.4 & 45.0 \\
%l5-ft & 57.8 & 63.9 & 38.8 & 28.0 & 29.0&54.8&66.9&51.3 & 30.5 & 52.1 & 45.2 & 43.2 & 57.3 & 58.8 & 46.0 & 27.2 & 51.2 & 39.3 & 53.3 & 56.6 & 47.6 \\
%\hline 
%l6-ft &63.5 & 66.3 & 48.7 & 38.1 & 30.6 & 61.4 & 70.9 & 60.3 & 34.8 & 57.8 & 47.6 & 53.6 & 59.8 & 63.5 & 52.5 & 29.8 & 54.6 & 48.2 & 58.5 & 62.2 & 53.1 \\
%l6-fc-ft& 61.4 & 63.9 & 44.2 & 36.2 & 29.0 & 59.9 & 66.0 & 55.3 & 31.1 & 57.6 & 49.5 & 49.4 & 59.4 & 63.7 & 50.8 & 29.5 & 54.1 & 43.2 & 57.4 & 58.8 & 51.0 \\
%\hline
%l7 & 57.6 & 57.2 & 41.4 & 31.2 & 25.6 & 52.4 & 58.8 & 50.9 & 25.2 & 50.4 & 42.7 & 47.1 & 52.2 & 55.6 & 44.5 & 23.9 & 48.0 & 38.1 & 51.5 & 56.6 & 45.5 \\
%l7-ft & 64.3 & 69.6 & 50.1 & 41.8 & 32.0 & 62.6 & 71.0 & 60.6 & 32.8 & 58.5 & 46.4 & 56.0 & 60.0 & 66.9 & 54.2 & 31.5 & 52.7 & 48.8 & 57.7 & 64.7 & 54.1 \\
%l7-fc-ft & 62.9 & 65.2 & 47.5 & 39.0 & 30.3 & 63.1 & 68.4 & 59.7 & 34.2 & 58.5 & 52.0 & 53.8 & 60.7 & 65.3 & 53.0 & 30.2 & 55.5 & 46.3 & 57.7 & 62.2 & 53.3 \\
%\hline
%\end{tabular}}
%\end{center}
%\end{table}
%\setlength{\tabcolsep}{1.4pt}

%A detailed layer-wise analysis of detection performance for all PASCAL classes and the 3 network configurations is presented in table \ref{table:det-fine}. %
%Notice that for both the finetuned networks there is big jump in the performance while going from layer 5 to 6 and a rather small jump from layer 6 to 7. For Alex-Net, the performance is virtually the same for layers 5 and 7. It is also notable, that although the performance for FT-net is better by 2.6 points at layer 5 - the performance is virtually the same at layer 7. 

%\subsection{Discussion}
%\label{sub:fine-discussion}
%Since layers 1-5 change a little over the course finetuning, this suggests that these are generic features. 
%
%%Although, one could always improve performance by a few points by finetuning the full network - for a lot of applications this may not be practical. 
%
%\todo{Talk about the entropy metric with respect to code being distributed.}
%
%\todo{Side Note - may or may not include}In our experiments we also noted accuracy of image classification on PASCAL is almost untouched by finetuning. This is suggestive of the fact finetuning is a task specific operation and finetuning for detection does not necessarily leads to an increase in classification performance, even though the classes and images are shared across PASCAL classification and detection challenges.

\subsection{Effect of pre-training on CNN parameters}
\label{sec:speed}
\input{texfiles/training_progress.tex}


==> texfiles/training_progress.tex <==
%\section{How does pre-training time affect generalization performance?}
%\label{sec:speed}
%Pre-Training is the process of initializing CNN parameters for a target application using images from a (generally larger) separate dataset. Features learned by a CNN pre-trained on Imagenet have been shown to generalize and achieve state of art results across multiple computer vision datasets (see section \ref{sec:fine} and \cite{Decaf}). Since, no single image dataset fully captures the variation in natural images, all datasets are biased (cite Alyosha). Consequently, it can be expected that excessive pre-training can cause the CNN to overfit on Imagenet and thus hurt generalization performance. 
There is no single image dataset that fully captures the variation in natural images. This means that all datasets, including ImageNet, are biased in some way. Thus, there is a possibility that pre-training may eventually cause the CNN to overfit and consequently hurt generalization performance \cite{torralba2011unbiased}. To understand if this happens, in the specific case of ImageNet pre-training, we investigated the effect of pre-training time on generalization performance both with and without fine-tuning. We find that pre-training for longer improves performance. This is surprising, as it shows that fitting more to ImageNet leads to better performance when moving to the other datasets that we evaluated.
%The other interesting thing we note is that within 50K iterations of pre-training, the performance is almost 90\% of the final performance achieved after nearly 300K iterations.

\setlength{\tabcolsep}{4pt}
\begin{table}[t!]
\begin{center}
\caption{Performance variation (\% mAP) on PASCAL-CLS as a function of pre-training iterations on ImageNet. The error bars  for all columns are similar to the one reported in the 305k column.}
\label{table:det-traj-classify}
\vspace{0.3em}
\begin{tabular}{lcccccccccc}
layer  & 5k & 15k & 25k & 35k & 50k & 95k & 105k & 195k & 205k & 305k \\
\hline
conv-1 & 23.0 & 24.3 & 24.4 & 24.5 & 24.3 & 24.8 & 24.7 & 24.4 & $24.4$  & $24.4 \pm 0.5$ \\
conv-2 & 33.7 & 40.4 & 40.9 & 41.8 & 42.7 & 43.2 & 44.0 & 45.0 & $45.1$  & $45.1 \pm 0.7$ \\
conv-3 & 34.2 & 46.8 & 47.0 & 48.2 & 48.6 & 49.4 & 51.6 & 50.7 & $50.9$  & $50.5 \pm 0.6$ \\
conv-4 & 33.5 & 49.0 & 48.7 & 50.2 & 50.7 & 51.6 & 54.1 & 54.3 & $54.4$  & $54.2 \pm 0.7$ \\
conv-5 & 33.0 & 53.4 & 55.0 & 56.8 & 57.3 & 59.2 & 63.5 & 64.9 & $65.5$  & $65.6 \pm 0.3 $ \\
fc-6   & 34.2 & 59.7 & 62.6 & 62.7 & 63.5 & 65.6 & 69.3 & 71.3 & $71.8$  & $72.1 \pm 0.3 $\\
fc-7   & 30.9 & 61.3 & 64.1 & 65.1 & 65.9 & 67.8 & 71.8 & 73.4 & $74.0$  & $74.3 \pm 0.3 $\\
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

We report performance on PASCAL-CLS as a function of pre-training time, without fine-tuning, in Table \ref{table:det-traj-classify}. Notice that more pre-training leads to better performance. By 15k and 50k iterations all layers are close to 80\% and  90\% of their final performance (5k iterations is only $\sim$1 epoch). This indicates that training required for generalization takes place quite quickly. Figure \ref{fig:conv1} shows conv-1 filters after 5k, 15k, and 305k iterations and reinforces this observation. Further, notice from Table \ref{table:det-traj-classify} that conv-1 trains first and the higher the layer is the more time it takes to converge. This suggests that a CNN, trained with backpropagation, converges in a layer-by-layer fashion.
Table \ref{table:det-trajectory} shows the interaction between varied amounts of pre-training time and fine-tuning on SUN-CLS and PASCAL-DET.
Here we also see that more pre-training prior to fine-tuning leads to better performance.

\begin{figure}[t!]
\centering
\subfloat[5k Iterations]{\includegraphics[scale=0.10]{l1_filters_iter5000.png}} \hspace{2mm}
\subfloat[15k Iterations]{\includegraphics[scale=0.10]{l1_filters_iter15000.png}} \hspace{2mm}
\subfloat[305k Iterations]{\includegraphics[scale=0.10]{l1_filters_iter225000.png}}
%\caption{(a), (b), and (c) show conv-1 filters after 5k, 15k and 305k iterations of training, respectively. Notice that after just 15k iterations these filters closely resemble their final state.}
\caption{Evolution of conv-1 filters with time. After just 15k iterations, these filters closely resemble their converged state.}
\begin{comment} Note: I have labeled 305k as 225k - I cannot get the same shape as of the 5k, 15k for 305k. The filters look very similar and visually indistinguishable from 305k. If I have time later, I will make them all uniform.
\end{comment}
\label{fig:conv1}
\end{figure}

\setlength{\tabcolsep}{4pt}
\begin{table}[t!]
\begin{center}
\caption{Performance variation on SUN-CLS and PASCAL-DET using features from a CNN pre-trained for different numbers of iterations and fine-tuned for a fixed number of iterations (40k for SUN-CLS and 70k for PASCAL-DET)}
\label{table:det-trajectory}
\vspace{0.3em}
\scalebox{1.00}{
\begin{tabular}{l|c|c|c|c}
 & 50k & 105k & 205k & 305k \\
\hline
\textbf{SUN-CLS} & $53.0 \pm 0.2 $ & $54.6 \pm 0.1 $ & $56.3 \pm 0.2 $ & $56.6 \pm 0.2$ \\
\textbf{PASCAL-DET} & 50.2 & 52.6 & 55.3 & 55.4\footnotemark \\
\end{tabular}}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt} 

\footnotetext{A network pre-trained from scratch, which was different from the one used in Section \ref{sub:fine-performance}, was used to obtain these results. The difference in performance is not significant.} 

